Bright low mass eclipsing binary candidates observed by STEREO

Observations from the Heliospheric Imagers (HI-1) on both the STEREO spacecraft have been analysed to search for bright low mass eclipsing binaries (EBs) and potential brown dwarf transits and to determine the radii of the companions. A total of 9 EB candidates have been found, ranging in brightness from V=6.59 mag to V=11.3 mag, where the radius of the companion appears to be less than 0.4 Rsol, with a diverse range of host temperatures, from 4074 K to 6925 K. Both components of one candidate, BD-07 3648, appear to be less than 0.4 Rsol and this represents a particularly interesting system for further study. The shapes of the eclipses in some cases are not clear enough to be certain they are total and the corresponding radii found should therefore be considered as lower limits. The EBs reported in this paper have either been newly found by the present analysis, or previously reported to be eclipsing by our earlier STEREO/HI-1 results. One of the new objects has subsequently been confirmed using archival SuperWASP data. This study was made possible by using an improved matched filter extraction algorithm, which is described in this paper.

==> authors.tex <==
\author[K. T. Wraight, L. Fossati, Glenn J. White, A. J. Norton and D. Bewsher]{{\textmd {\textbf }}\\
    \textup{K.T. Wraight}$^1$, \textup{L. Fossati}$^{1}$, \textup{Glenn J. White}$^{1,2}$, \textup{A.J. Norton}$^1$ \textup{and} \textup{D. Bewsher}$^3$\\    
    $^1$\textit{Department of Physics and Astronomy, The Open University, Milton Keynes, MK7 6AA, UK}\\
    $^2$\textit{Space Science and Technology Department, STFC Rutherford Appleton Laboratory, Chilton, Didcot, Oxfordshire, OX11 0QX, UK}\\
    $^3$\textit{Jeremiah Horrocks Institute, University of Central Lancashire, Preston, Lancashire, PR1 2HE, UK}\\
}
